Pivot Through English: Reliably Answering Multilingual Questions without Document Retrieval

Existing methods for open-retrieval question answering in lower resource languages (LRLs) lag significantly behind English. They not only suffer from the shortcomings of non-English document retrieval, but are reliant on language-specific supervision for either the task or translation. We formulate a task setup more realistic to available resources, that circumvents document retrieval to reliably transfer knowledge from English to lower resource languages. Assuming a strong English question answering model or database, we compare and analyze methods that pivot through English: to map foreign queries to English and then English answers back to target language answers. Within this task setup we propose Reranked Multilingual Maximal Inner Product Search (RM-MIPS), akin to semantic similarity retrieval over the English training set with reranking, which outperforms the strongest baselines by 2.7% on XQuAD and 6.2% on MKQA. Analysis demonstrates the particular efficacy of this strategy over state-of-the-art alternatives in challenging settings: low-resource languages, with extensive distractor data and query distribution misalignment. Circumventing retrieval, our analysis shows this approach offers rapid answer generation to almost any language off-the-shelf, without the need for any additional training data in the target language.

==> tables/paraphrase_detection.tex <==
\begin{table}[htp] % htp
\centering
\begin{small}
\begin{tabular}{l|cc}
% \toprule
% %  \multicolumn{2}{c}{XLM-R Accuracy} \\
% QQP & PAWS-X \\
%  \midrule
% & \\
% \bottomrule
\toprule
Method & QQP & PAWS-X \\\midrule
NMT + USE & 0.570 & 0.581 \\
LASER & 0.640 & 0.637 \\
mUSE & 0.562 & 0.597 \\
Dual Encoder (XLM-R) & 0.644 & 0.623 \\
% SBERT XLM-R & 0.875 & 0.820 \\
XLM-R & & \\\hline
\textit{SOTA} & & \\
\bottomrule
\end{tabular}
\end{small}
\caption{The accuracies on the test sets of XLM-R trained on 75\% PAWS-X and 25\% QQP}
\end{table}


% Method & QQP & PAWS-X \\hline
% nmt-zero-L24-RoBT-use-large & 0.570 & 0.554 \\
% umlpd-laser & 0.640 & 0.599 \\
% umlpd-muse-large & 0.562 & 0.567 \\
% umlpd-sbertm & 0.644 & 0.583 \\
% umlpd-sbert-xlmr-75-25 & 0.875 & 0.805 \\

==> tables/xxen_mkqa_1.tex <==

\begin{table*}[]
\centering
\begin{tabular}{lccccccccccc}
\toprule
 & \multicolumn{10}{c}{XX $\rightarrow$ EN (1/3)} \\
\cmidrule{2-12}
 & \multicolumn{1}{|l|}{avg} & ar & da & de & es & fi & fr & he & hu & it & ja\\
\midrule
NMT USE-L & \multicolumn{1}{|l|}{0.84} & 0.80 & 0.95 & 0.94 & 0.93 & 0.86 & 0.94 & 0.85 & 0.89 & 0.93 & 0.75 \\\hline
LASER & \multicolumn{1}{|l|}{0.82} & 0.90 & 0.93 & 0.58 & 0.87 & 0.89 & 0.86 & 0.92 & 0.78 & 0.87 & 0.51 \\
MUSE-L & \multicolumn{1}{|l|}{0.79} & 0.89 & 0.65 & 0.96 & 0.97 & 0.48 & 0.96 & 0.32 & 0.51 & 0.96 & 0.89 \\
SBERT XLM-R & \multicolumn{1}{|l|}{0.51} & 0.36 & 0.72 & 0.60 & 0.57 & 0.50 & 0.61 & 0.41 & 0.44 & 0.57 & 0.30 \\
XLM-R & \multicolumn{1}{|l|}{\textbf{0.77}} & 0.68 & 0.84 & 0.79 & 0.81 & 0.76 & 0.81 & 0.74 & 0.73 & 0.80 & 0.72 \\
XLM-R (75, 25) & \multicolumn{1}{|l|}{\textbf{0.91}} & 0.83 & 0.95 & 0.93 & 0.94 & 0.91 & 0.92 & 0.89 & 0.90 & 0.92 & 0.88 \\
XLM-R (50, 50) & \multicolumn{1}{|l|}{0.79} & 0.63 & 0.90 & 0.86 & 0.85 & 0.73 & 0.87 & 0.71 & 0.72 & 0.81 & 0.71 \\
SBERT XLM-R (75, 25) & \multicolumn{1}{|l|}{0.81} & 0.63 & 0.92 & 0.88 & 0.88 & 0.76 & 0.87 & 0.73 & 0.78 & 0.83 & 0.77 \\
Hybrid XLM-R (k=4) & \multicolumn{1}{|l|}{0.85} & 0.70 & 0.94 & 0.91 & 0.91 & 0.82 & 0.90 & 0.79 & 0.83 & 0.87 & 0.82 \\
Hybrid XLM-R (k=8) & \multicolumn{1}{|l|}{0.87} & 0.73 & 0.94 & 0.92 & 0.92 & 0.84 & 0.91 & 0.82 & 0.84 & 0.88 & 0.84 \\
Hybrid XLM-R (k=16) & \multicolumn{1}{|l|}{0.88} & 0.75 & 0.95 & 0.93 & 0.92 & 0.85 & 0.92 & 0.84 & 0.86 & 0.89 & 0.85 \\
Hybrid XLM-R (k=32) & \multicolumn{1}{|l|}{0.89} & 0.77 & 0.95 & 0.93 & 0.93 & 0.87 & 0.92 & 0.85 & 0.87 & 0.90 & 0.86 \\
Hybrid XLM-R (k=64) & \multicolumn{1}{|l|}{0.90} & 0.78 & 0.95 & 0.93 & 0.93 & 0.88 & 0.93 & 0.87 & 0.88 & 0.91 & 0.87 \\
Hybrid XLM-R (k=128) & \multicolumn{1}{|l|}{0.90} & 0.80 & 0.95 & 0.94 & 0.94 & 0.89 & 0.93 & 0.88 & 0.89 & 0.92 & 0.88 \\
Hybrid XLM-R (k=256) & \multicolumn{1}{|l|}{\textbf{0.91}} & 0.82 & 0.96 & 0.94 & 0.94 & 0.90 & 0.93 & 0.88 & 0.89 & 0.92 & 0.88 \\
Hybrid XLM-R (k=512) & \multicolumn{1}{|l|}{\textbf{0.91}} & 0.83 & 0.96 & 0.94 & 0.94 & 0.90 & 0.93 & 0.89 & 0.90 & 0.93 & 0.88 \\
Hybrid XLM-R (k=1024) & \multicolumn{1}{|l|}{\textbf{0.91}} & 0.83 & 0.96 & 0.94 & 0.94 & 0.91 & 0.93 & 0.90 & 0.90 & 0.93 & 0.89 \\
\bottomrule
\end{tabular}
\caption{MKQA XX $\rightarrow$ EN Accuracies (1/3)}
\end{table*}

% NMT USE-L	0.84
% LASER	0.82
% MUSE-L	0.79
% SBERT XLM-R	0.51
% XLM-R	0.77
% XLM-R (75, 25)	0.91
% XLM-R (50, 50)	0.79
% SBERT XLM-R (75, 25)	0.81
% Hybrid XLM-R (k=4)	0.85
% Hybrid XLM-R (k=8)	0.87
% Hybrid XLM-R (k=16)	0.88
% Hybrid XLM-R (k=32)	0.89
% Hybrid XLM-R (k=64)	0.90
% Hybrid XLM-R (k=128	0.90
% Hybrid XLM-R (k=256)	0.91
% Hybrid XLM-R (k=512)	0.91
% Hybrid XLM-R (k=1024)	0.91
% avg ar da de es fi fr he hu it ja



% \begin{table*}[]
% \centering
% \begin{tabular}{}

% \end{tabular}
% \caption{MKQA XX $\rightarrow$ EN Accuracies (1/3)}
% \end{table*}

==> tables/xxen_mkqa_2.tex <==

\begin{table*}[]
\centering
\begin{tabular}{lccccccccccc}
\toprule
 & \multicolumn{10}{c}{EN $\rightarrow$ XX (2/3)} \\
\cmidrule{2-12}
 & km & ms & nl & no & pl & pt & ru & sv & th & tr & vi \\
\midrule
NMT USE-L & 0.55 & 0.93 & 0.95 & 0.93 & 0.90 & 0.94 & 0.90 & 0.94 & 0.86 & 0.89 & 0.87 \\\hline
LASER & 0.45 & 0.97 & 0.97 & 0.96 & 0.83 & 0.90 & 0.87 & 0.96 & 0.73 & 0.85 & 0.89 \\
MUSE-L & 0.44 & 0.95 & 0.97 & 0.63 & 0.93 & 0.97 & 0.94 & 0.64 & 0.95 & 0.94 & 0.41 \\
SBERT XLM-R & 0.40 & 0.64 & 0.72 & 0.71 & 0.53 & 0.64 & 0.51 & 0.71 & 0.50 & 0.37 & 0.52 \\
XLM-R & 0.71 & 0.82 & 0.83 & 0.83 & 0.78 & 0.82 & 0.80 & 0.84 & 0.79 & 0.78 & 0.75 \\
XLM-R (75, 25) & 0.83 & 0.95 & 0.93 & 0.94 & 0.92 & 0.93 & 0.92 & 0.95 & 0.93 & 0.91 & 0.92 \\
XLM-R (50, 50) & 0.68 & 0.83 & 0.88 & 0.88 & 0.78 & 0.86 & 0.81 & 0.89 & 0.80 & 0.70 & 0.79 \\
SBERT XLM-R (75, 25) & 0.60 & 0.88 & 0.91 & 0.90 & 0.84 & 0.86 & 0.84 & 0.91 & 0.85 & 0.72 & 0.82 \\
Hybrid XLM-R (k=4) & 0.67 & 0.91 & 0.93 & 0.92 & 0.88 & 0.89 & 0.88 & 0.93 & 0.89 & 0.78 & 0.86 \\
Hybrid XLM-R (k=8) & 0.70 & 0.92 & 0.94 & 0.93 & 0.89 & 0.91 & 0.89 & 0.94 & 0.90 & 0.80 & 0.88 \\
Hybrid XLM-R (k=16) & 0.72 & 0.93 & 0.94 & 0.93 & 0.90 & 0.92 & 0.90 & 0.94 & 0.91 & 0.82 & 0.89 \\
Hybrid XLM-R (k=32) & 0.74 & 0.94 & 0.95 & 0.94 & 0.91 & 0.93 & 0.91 & 0.95 & 0.92 & 0.84 & 0.90 \\
Hybrid XLM-R (k=64) & 0.76 & 0.94 & 0.95 & 0.94 & 0.92 & 0.93 & 0.92 & 0.95 & 0.92 & 0.85 & 0.91 \\
Hybrid XLM-R (k=128 & 0.78 & 0.95 & 0.95 & 0.94 & 0.92 & 0.94 & 0.92 & 0.96 & 0.93 & 0.87 & 0.91 \\
Hybrid XLM-R (k=256) & 0.80 & 0.95 & 0.95 & 0.95 & 0.92 & 0.94 & 0.93 & 0.96 & 0.93 & 0.88 & 0.92 \\
Hybrid XLM-R (k=512) & 0.81 & 0.95 & 0.95 & 0.95 & 0.93 & 0.94 & 0.93 & 0.96 & 0.93 & 0.89 & 0.92 \\
Hybrid XLM-R (k=1024) & 0.82 & 0.96 & 0.95 & 0.95 & 0.93 & 0.94 & 0.93 & 0.96 & 0.93 & 0.90 & 0.93 \\
\bottomrule
\end{tabular}
\caption{MKQA XX $\rightarrow$ EN Accracies (2/3)}
\end{table*} 

==> tables/xxen_mkqa_3.tex <==

\begin{table*}[]
\centering
\begin{tabular}{lccc}
\toprule
 & \multicolumn{3}{c}{EN $\rightarrow$ XX (3/3)} \\
\cmidrule{2-4}
 & zh-cn & zh-hk & zh-tw \\
\midrule
NMT USE-L & 0.62 & 0.55 & 0.51 \\\hline
LASER & 0.76 & 0.77 & 0.71 \\
MUSE-L & 0.92 & 0.90 & 0.85 \\
SBERT XLM-R & 0.31 & 0.36 & 0.30 \\
XLM-R & 0.70 & 0.71 & 0.63 \\
XLM-R (75, 25) & 0.88 & 0.87 & 0.82 \\
XLM-R (50, 50) & 0.77 & 0.77 & 0.71 \\
SBERT XLM-R (75, 25) & 0.79 & 0.78 & 0.73 \\
Hybrid XLM-R (k=4) & 0.84 & 0.83 & 0.78 \\
Hybrid XLM-R (k=8) & 0.86 & 0.84 & 0.79 \\
Hybrid XLM-R (k=16) & 0.87 & 0.85 & 0.81 \\
Hybrid XLM-R (k=32) & 0.88 & 0.86 & 0.82 \\
Hybrid XLM-R (k=64) & 0.88 & 0.87 & 0.82 \\
Hybrid XLM-R (k=128 & 0.88 & 0.87 & 0.83 \\
Hybrid XLM-R (k=256) & 0.89 & 0.88 & 0.83 \\
Hybrid XLM-R (k=512) & 0.89 & 0.88 & 0.83 \\
Hybrid XLM-R (k=1024) & 0.89 & 0.88 & 0.83 \\
\bottomrule
\end{tabular}
\caption{MKQA XX $\rightarrow$ EN Accuracies (3/3)}
\end{table*}

==> tables/xxen_partial.tex <==

\begin{table*}[htbp]
\centerline{
\begin{tabular}{lccccccccccc}
\toprule
 & \multicolumn{10}{c}{XQuAD + SQuAD} \\
\cmidrule{2-12}
 & \multicolumn{1}{|c|}{avg} & ar & de & el & es & hi & ru & th & tr & vi & zh \\
\midrule

NMT + USE & \multicolumn{1}{|c|}{0.77 \pm 0.15} & 0.95 & 0.91 & 0.86 & 0.85 & 0.82 & 0.79 & 0.74 & 0.71 & 0.67 & 0.41 \\
mUSE & \multicolumn{1}{|c|}{0.68 \pm 0.39} & \textbf{0.98} & \textbf{0.96} & 0.07 & \textbf{0.93} & \textbf{0.94} & 0.03 & 0.17 & \textbf{0.87} & \textbf{0.91} & \textbf{0.90} \\
LASER & \multicolumn{1}{|c|}{0.46 \pm 0.25} & 0.86 & 0.33 & 0.03 & 0.70 & 0.65 & 0.28 & 0.64 & 0.61 & 0.24 & 0.29 \\
S-BERT & \multicolumn{1}{|c|}{0.81 \pm 0.06} & 0.87 & 0.85 & 0.81 & 0.85 & 0.81 & 0.77 & 0.89 & 0.66 & 0.76 & 0.82 \\
S-BERT XLM-R & \multicolumn{1}{|c|}{0.78 \pm 0.10} & 0.93 & 0.90 & 0.79 & 0.82 & 0.81 & 0.72 & 0.85 & 0.62 & 0.60 & 0.75 \\
Hybrid XLM-R (k=64) & \multicolumn{1}{|c|}{0.89 \pm 0.05} & 0.96 & 0.95 & \textbf{0.91} & 0.91 & 0.91 & \textbf{0.89} & 0.91 & 0.81 & 0.80 & 0.87 \\
% Hybrid XLM-R (k=32) & \multicolumn{1}{|c|}{0.89 \pm 0.06} & 0.96 & 0.95 & 0.90 & 0.91 & 0.91 & 0.87 & \textbf{0.92} & 0.79 & 0.77 & 0.86 \\
% Hybrid XLM-R (k=16) & \multicolumn{1}{|c|}{0.87 \pm 0.07} & 0.96 & 0.95 & 0.89 & 0.89 & 0.89 & 0.84 & 0.91 & 0.76 & 0.75 & 0.85 \\
% Hybrid XLM-R (k=8) & \multicolumn{1}{|c|}{0.85 \pm 0.08} & 0.94 & 0.94 & 0.87 & 0.89 & 0.88 & 0.81 & 0.91 & 0.73 & 0.71 & 0.83 \\
% Hybrid XLM-R (k=4) & \multicolumn{1}{|c|}{0.83 \pm 0.08} & 0.94 & 0.94 & 0.84 & 0.87 & 0.87 & 0.79 & 0.89 & 0.70 & 0.68 & 0.81 \\



% NMT + USE & \multicolumn{1}{|c|}{0.77} & 0.71 & 0.91 & 0.86 & 0.95 & 0.79 & 0.85 & 0.67 & 0.82 & 0.74 & 0.41 \\\hline
% mUSE & \multicolumn{1}{|c|}{0.68} & \textbf{0.87} & \textbf{0.96} & 0.07 & \textbf{0.98} & 0.03 & \textbf{0.93} & \textbf{0.91} & \textbf{0.94} & 0.17 & \textbf{0.90} \\
% LASER & \multicolumn{1}{|c|}{0.46} & 0.61 & 0.33 & 0.03 & 0.86 & 0.28 & 0.70 & 0.24 & 0.65 & 0.64 & 0.29 \\
% S-BERT & \multicolumn{1}{|c|}{0.81} & 0.66 & 0.85 & 0.81 & 0.87 & 0.77 & 0.85 & 0.76 & 0.81 & 0.89 & 0.82 \\
% S-BERT XLM-R & \multicolumn{1}{|c|}{0.78} & 0.62 & 0.90 & 0.79 & 0.93 & 0.72 & 0.82 & 0.60 & 0.81 & 0.85 & 0.75 \\
% Hybrid XLM-R (k=64) & \multicolumn{1}{|c|}{\textbf{0.89}} & 0.81 & 0.95 & \textbf{0.91} & 0.96 & \textbf{0.89} & 0.91 & 0.80 & 0.91 & \textbf{0.91} & 0.87 \\
\toprule
 & \multicolumn{10}{c}{MKQA + Natural Questions} \\
\cmidrule{2-12}
 & \multicolumn{1}{|c|}{avg} & da & nl & fr & pt & de & ar & ja & ko & km & $zh_{tw}$ \\
\midrule

NMT + USE & \multicolumn{1}{|c|}{0.73 \pm 0.16} & \textbf{0.89} & 0.88 & 0.87 & 0.87 & 0.87 & 0.68 & 0.61 & 0.53 & 0.45 & 0.39 \\
mUSE & \multicolumn{1}{|c|}{0.71 \pm 0.21} & 0.51 & 0.91 & \textbf{0.91} & \textbf{0.93} & \textbf{0.90} & 0.79 & \textbf{0.79} & \textbf{0.73} & 0.35 & \textbf{0.72} \\
LASER & \multicolumn{1}{|c|}{0.73 \pm 0.15} & 0.88 & \textbf{0.93} & 0.78 & 0.84 & 0.52 & \textbf{0.81} & 0.39 & 0.68 & 0.40 & 0.57 \\
S-BERT & \multicolumn{1}{|c|}{0.72 \pm 0.07} & 0.84 & 0.78 & 0.73 & 0.65 & 0.74 & 0.57 & 0.70 & 0.71 & 0.58 & 0.70 \\
S-BERT XLM-R & \multicolumn{1}{|c|}{0.70 \pm 0.10} & 0.85 & 0.83 & 0.77 & 0.76 & 0.79 & 0.51 & 0.64 & 0.60 & 0.49 & 0.60 \\
Hybrid XLM-R (k=64) & \multicolumn{1}{|c|}{0.79 \pm 0.07} & 0.88 & 0.88 & 0.85 & 0.85 & 0.85 & 0.66 & 0.75 & 0.69 & \textbf{0.63} & 0.70 \\
% Hybrid XLM-R (k=32) & \multicolumn{1}{|c|}{0.79 \pm 0.07} & 0.88 & 0.87 & 0.84 & 0.84 & 0.85 & 0.64 & 0.74 & 0.69 & 0.62 & 0.70 \\
% Hybrid XLM-R (k=16) & \multicolumn{1}{|c|}{0.78 \pm 0.07} & 0.88 & 0.87 & 0.84 & 0.84 & 0.85 & 0.63 & 0.73 & 0.69 & 0.60 & 0.69 \\
% Hybrid XLM-R (k=8) & \multicolumn{1}{|c|}{0.77 \pm 0.08} & 0.88 & 0.87 & 0.83 & 0.83 & 0.84 & 0.62 & 0.72 & 0.69 & 0.59 & 0.69 \\
% Hybrid XLM-R (k=4) & \multicolumn{1}{|c|}{0.76 \pm 0.08} & 0.87 & 0.86 & 0.83 & 0.82 & 0.84 & 0.60 & 0.71 & 0.68 & 0.58 & 0.68 \\




% NMT + USE & \multicolumn{1}{|c|}{0.73} & \textbf{0.89} & 0.88 & 0.87 & 0.87 & 0.87 & 0.68 & 0.61 & 0.53 & 0.45 & 0.39 \\\hline
% mUSE & \multicolumn{1}{|c|}{0.71} & 0.51 & 0.91 & \textbf{0.91} & \textbf{0.93} & \textbf{0.90} & 0.79 & \textbf{0.79} & \textbf{0.73} & 0.35 & \textbf{0.72} \\
% LASER & \multicolumn{1}{|c|}{0.73} & 0.88 & \textbf{0.93} & 0.78 & 0.84 & 0.52 & \textbf{0.81} & 0.39 & 0.68 & 0.40 & 0.57 \\
% S-BERT & \multicolumn{1}{|c|}{0.72} & 0.84 & 0.78 & 0.73 & 0.65 & 0.74 & 0.57 & 0.70 & 0.71 & 0.58 & 0.70 \\
% S-BERT XLM-R & \multicolumn{1}{|c|}{0.70} & 0.85 & 0.83 & 0.77 & 0.76 & 0.79 & 0.51 & 0.64 & 0.60 & 0.49 & 0.60 \\
% Hybrid XLM-R (k=64) & \multicolumn{1}{|c|}{\textbf{0.79}} & 0.88 & 0.88 & 0.85 & 0.85 & 0.85 & 0.66 & 0.75 & 0.69 & \textbf{0.63} & 0.70 \\
% % Hybrid XLM-R (k=32) & \multicolumn{1}{|c|}{0.79} & 0.88 & 0.87 & 0.84 & 0.84 & 0.85 & 0.64 & 0.74 & 0.69 & 0.62 & 0.70 \\
% % Hybrid XLM-R (k=16) & \multicolumn{1}{|c|}{0.78} & 0.88 & 0.87 & 0.84 & 0.84 & 0.85 & 0.63 & 0.73 & 0.69 & 0.60 & 0.69 \\
% % Hybrid XLM-R (k=8) & \multicolumn{1}{|c|}{0.77} & 0.88 & 0.87 & 0.83 & 0.83 & 0.84 & 0.62 & 0.72 & 0.69 & 0.59 & 0.69 \\
% % Hybrid XLM-R (k=4) & \multicolumn{1}{|c|}{0.76} & 0.87 & 0.86 & 0.83 & 0.82 & 0.84 & 0.60 & 0.71 & 0.68 & 0.58 & 0.68 \\
%  & \multicolumn{1}{|c|}{avg} & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ \\
% \midrule
% \_\_ & \multicolumn{1}{|c|}{\_\_} & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ \\\hline
% \_\_ & \multicolumn{1}{|c|}{\_\_} & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ \\
% \_\_ & \multicolumn{1}{|c|}{\_\_} & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ \\
% \_\_ & \multicolumn{1}{|c|}{\_\_} & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ \\
% \_\_ & \multicolumn{1}{|c|}{\_\_} & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ \\
% \_\_ & \multicolumn{1}{|c|}{\_\_} & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ \\

% \bottomrule
% \toprule
%  & \multicolumn{10}{c}{MKQA} \\
% \cmidrule{2-13}
%  & \multicolumn{1}{|c}{avg} & \multicolumn{1}{c|}{std} & ar & da & de & es & fi & fr & he & hu & it & ja\\
% \midrule
% NMT USE-L & \multicolumn{1}{|l}{0.82} & \multicolumn{1}{l|}{0.093} & 0.80 & \textbf{0.95} & 0.94 & 0.93 & 0.86 & 0.94 & 0.85 & 0.89 & 0.93 & 0.75 \\\hline
% LASER & \multicolumn{1}{|l}{0.79} & \multicolumn{1}{l|}{0.260} & \textbf{0.90} & 0.93 & 0.58 & 0.87 & 0.89 & 0.86 & \textbf{0.92} & 0.78 & 0.87 & 0.51 \\
% MUSE-L & \multicolumn{1}{|l}{0.51} & \multicolumn{1}{l|}{0.395} & 0.89 & 0.65 & \textbf{0.96} & \textbf{0.97} & 0.48 & \textbf{0.96} & 0.32 & 0.51 & \textbf{0.96} & \textbf{0.89} \\
% XLM-R & \multicolumn{1}{|l}{\textbf{0.91}} & \multicolumn{1}{l|}{\textbf{0.014}} & 0.83 & \textbf{0.95} & 0.93 & \textbf{0.94} & \textbf{0.91} & 0.92 & 0.89 & \textbf{0.90} & 0.92 & 0.88 \\
% SBERT XLM-R & \multicolumn{1}{|l}{0.85} & \multicolumn{1}{l|}{0.057} & 0.63 & 0.92 & 0.88 & 0.88 & 0.76 & 0.87 & 0.73 & 0.78 & 0.83 & 0.77 \\
% Hybrid XLM-R & \multicolumn{1}{|l}{\textbf{0.91}} & \multicolumn{1}{l|}{\textbf{0.014}} & 0.78 & \textbf{0.95} & 0.93 & 0.93 & 0.88 & 0.93 & 0.87 & 0.88 & 0.91 & 0.87 \\
\bottomrule

\end{tabular}}
\caption{XX $\rightarrow$ EN Accuracies: The average accuracies obtained for each method on mapping from queries in a given language to English. Only a subset of the MQKA langauge results are shown: 5 of the languages NMT + USE performs the best, and 5 which it is least performant.}
\end{table*}




% \begin{table*}[htbp]
% \centering
% \begin{tabular}{lcccccccccccc}
% \toprule
%  & \multicolumn{10}{c}{XQuAD} \\
% \cmidrule{2-13}
%  & \multicolumn{1}{|c}{avg} & \multicolumn{1}{c|}{std} & ar & da & de & es & fi & fr & he & hu & it & ja\\
% \midrule
% NMT USE-L & \multicolumn{1}{|l}{0.82} & \multicolumn{1}{l|}{0.093} & 0.80 & \textbf{0.95} & 0.94 & 0.93 & 0.86 & 0.94 & 0.85 & 0.89 & 0.93 & 0.75 \\\hline
% LASER & \multicolumn{1}{|l}{0.79} & \multicolumn{1}{l|}{0.260} & \textbf{0.90} & 0.93 & 0.58 & 0.87 & 0.89 & 0.86 & \textbf{0.92} & 0.78 & 0.87 & 0.51 \\
% MUSE-L & \multicolumn{1}{|l}{0.51} & \multicolumn{1}{l|}{0.395} & 0.89 & 0.65 & \textbf{0.96} & \textbf{0.97} & 0.48 & \textbf{0.96} & 0.32 & 0.51 & \textbf{0.96} & \textbf{0.89} \\
% XLM-R & \multicolumn{1}{|l}{\textbf{0.91}} & \multicolumn{1}{l|}{\textbf{0.014}} & 0.83 & \textbf{0.95} & 0.93 & \textbf{0.94} & \textbf{0.91} & 0.92 & 0.89 & \textbf{0.90} & 0.92 & 0.88 \\
% SBERT XLM-R & \multicolumn{1}{|l}{0.85} & \multicolumn{1}{l|}{0.057} & 0.63 & 0.92 & 0.88 & 0.88 & 0.76 & 0.87 & 0.73 & 0.78 & 0.83 & 0.77 \\
% Hybrid XLM-R & \multicolumn{1}{|l}{\textbf{0.91}} & \multicolumn{1}{l|}{\textbf{0.014}} & 0.78 & \textbf{0.95} & 0.93 & 0.93 & 0.88 & 0.93 & 0.87 & 0.88 & 0.91 & 0.87 \\
% % \bottomrule
% \toprule
%  & \multicolumn{10}{c}{MKQA} \\
% \cmidrule{2-13}
%  & \multicolumn{1}{|c}{avg} & \multicolumn{1}{c|}{std} & ar & da & de & es & fi & fr & he & hu & it & ja\\
% \midrule
% % NMT USE-L & \multicolumn{1}{|l}{0.82} & \multicolumn{1}{l|}{0.093} & 0.80 & \textbf{0.95} & 0.94 & 0.93 & 0.86 & 0.94 & 0.85 & 0.89 & 0.93 & 0.75 \\\hline
% % LASER & \multicolumn{1}{|l}{0.79} & \multicolumn{1}{l|}{0.260} & \textbf{0.90} & 0.93 & 0.58 & 0.87 & 0.89 & 0.86 & \textbf{0.92} & 0.78 & 0.87 & 0.51 \\
% % MUSE-L & \multicolumn{1}{|l}{0.51} & \multicolumn{1}{l|}{0.395} & 0.89 & 0.65 & \textbf{0.96} & \textbf{0.97} & 0.48 & \textbf{0.96} & 0.32 & 0.51 & \textbf{0.96} & \textbf{0.89} \\
% % XLM-R & \multicolumn{1}{|l}{\textbf{0.91}} & \multicolumn{1}{l|}{\textbf{0.014}} & 0.83 & \textbf{0.95} & 0.93 & \textbf{0.94} & \textbf{0.91} & 0.92 & 0.89 & \textbf{0.90} & 0.92 & 0.88 \\
% % SBERT XLM-R & \multicolumn{1}{|l}{0.85} & \multicolumn{1}{l|}{0.057} & 0.63 & 0.92 & 0.88 & 0.88 & 0.76 & 0.87 & 0.73 & 0.78 & 0.83 & 0.77 \\
% % Hybrid XLM-R & \multicolumn{1}{|l}{\textbf{0.91}} & \multicolumn{1}{l|}{\textbf{0.014}} & 0.78 & \textbf{0.95} & 0.93 & 0.93 & 0.88 & 0.93 & 0.87 & 0.88 & 0.91 & 0.87 \\
% \bottomrule

% \end{tabular}
% \caption{XX $\rightarrow$ EN Accuracies: Probably will replace these with distractor data}
% \end{table*}

















% \toprule
%  & \multicolumn{10}{c}{XQuAD XX $\rightarrow$ EN Accuracies} \\
% \cmidrule{2-13}
%  & \multicolumn{1}{|c}{avg} & \multicolumn{1}{c|}{std} & ar & da & de & es & fi & fr & he & hu & it & ja\\
% \midrule
% NMT USE-L & \multicolumn{1}{|l}{0.82} & \multicolumn{1}{l|}{0.093} & 0.80 & \textbf{0.95} & 0.94 & 0.93 & 0.86 & 0.94 & 0.85 & 0.89 & 0.93 & 0.75 \\\hline
% LASER & \multicolumn{1}{|l}{0.79} & \multicolumn{1}{l|}{0.260} & \textbf{0.90} & 0.93 & 0.58 & 0.87 & 0.89 & 0.86 & \textbf{0.92} & 0.78 & 0.87 & 0.51 \\
% MUSE-L & \multicolumn{1}{|l}{0.51} & \multicolumn{1}{l|}{0.395} & 0.89 & 0.65 & \textbf{0.96} & \textbf{0.97} & 0.48 & \textbf{0.96} & 0.32 & 0.51 & \textbf{0.96} & \textbf{0.89} \\
% XLM-R & \multicolumn{1}{|l}{\textbf{0.91}} & \multicolumn{1}{l|}{\textbf{0.014}} & 0.83 & \textbf{0.95} & 0.93 & \textbf{0.94} & \textbf{0.91} & 0.92 & 0.89 & \textbf{0.90} & 0.92 & 0.88 \\
% SBERT XLM-R & \multicolumn{1}{|l}{0.85} & \multicolumn{1}{l|}{0.057} & 0.63 & 0.92 & 0.88 & 0.88 & 0.76 & 0.87 & 0.73 & 0.78 & 0.83 & 0.77 \\
% Hybrid XLM-R & \multicolumn{1}{|l}{\textbf{0.91}} & \multicolumn{1}{l|}{\textbf{0.014}} & 0.78 & \textbf{0.95} & 0.93 & 0.93 & 0.88 & 0.93 & 0.87 & 0.88 & 0.91 & 0.87 \\
% \bottomrule


% \midrule
% NMT USE-L & \multicolumn{1}{|l|}{0.82} & 0.80 & \textbf{0.95} & 0.94 & 0.93 & 0.86 & 0.94 & 0.85 & 0.89 & 0.93 & 0.75 \\\hline
% LASER & \multicolumn{1}{|l|}{0.79} & \textbf{0.90} & 0.93 & 0.58 & 0.87 & 0.89 & 0.86 & \textbf{0.92} & 0.78 & 0.87 & 0.51 \\
% MUSE-L & \multicolumn{1}{|l|}{0.51} & 0.89 & 0.65 & \textbf{0.96} & \textbf{0.97} & 0.48 & \textbf{0.96} & 0.32 & 0.51 & \textbf{0.96} & \textbf{0.89} \\
% XLM-R & \multicolumn{1}{|l|}{\textbf{0.91}} & 0.83 & \textbf{0.95} & 0.93 & \textbf{0.94} & \textbf{0.91} & 0.92 & 0.89 & \textbf{0.90} & 0.92 & 0.88 \\
% SBERT XLM-R & \multicolumn{1}{|l|}{0.85} & 0.63 & 0.92 & 0.88 & 0.88 & 0.76 & 0.87 & 0.73 & 0.78 & 0.83 & 0.77 \\
% Hybrid XLM-R & \multicolumn{1}{|l|}{\textbf{0.91}} & 0.78 & \textbf{0.95} & 0.93 & 0.93 & 0.88 & 0.93 & 0.87 & 0.88 & 0.91 & 0.87 \\
% \bottomrule





% \begin{tabular}{l|cc|cc|}
% \toprule
% \multicolumn{1}{l|}{EN $\rightarrow$ XX} & \multicolumn{2}{c|}{XQuAD} & \multicolumn{2}{c|}{MKQA} \\
% \cmidrule{2-5}
% Model & Avg. Lang. Acc. & Speedup & Avg. Lang. Acc. & Speedup \\
% \midrule
% NMT + USE    & 0.82 &  &  & \\
% mUSE         &  &  &  & \\
% LASER        &  &  &  & \\
% S-BERT       &  &  &  & \\
% XLM-R        &  &  &  & \\
% S-XLM-R      &  &  &  & \\
% XLM-R Hybrid &  &  &  & \\
% \bottomrule

==> tables/xxen_partial_groups.tex <==

\begin{table*}[htbp]
\begin{small}
\begin{tabular}{l |c|ccc |c|ccc|}
\toprule
\multicolumn{1}{c}{} & \multicolumn{4}{|c|}{XQuAD + SQuAD} & \multicolumn{4}{|c|}{MKQA + Natural Questions} \\
\cmidrule{2-9}
 & Avg & High & Medium & Low & Avg & High & Medium & Low \\
\midrule

NMT + USE & 0.73 $\pm$ 0.16 & 0.78 $\pm$ 0.13 & 0.77 $\pm$ 0.10 & 0.57 $\pm$ 0.19 & 0.77 $\pm$ 0.15 & 0.78 $\pm$ 0.22 & 0.76 $\pm$ 0.05 & 0.78 $\pm$ 0.08 \\\hline
mUSE & 0.71 $\pm$ 0.21 & \textbf{0.87} $\pm$ 0.05 & 0.57 $\pm$ 0.20 & 0.72 $\pm$ 0.19 & 0.68 $\pm$ 0.39 & \textbf{0.94} $\pm$ 0.03 & 0.66 $\pm$ 0.35 & 0.34 $\pm$ 0.41 \\
LASER & 0.73 $\pm$ 0.15 & 0.69 $\pm$ 0.14 & 0.82 $\pm$ 0.09 & 0.63 $\pm$ 0.17 & 0.46 $\pm$ 0.25 & 0.54 $\pm$ 0.24 & 0.64 $\pm$ 0.02 & 0.18 $\pm$ 0.11 \\
S-BERT & 0.72 $\pm$ 0.07 & 0.72 $\pm$ 0.04 & 0.72 $\pm$ 0.08 & 0.71 $\pm$ 0.07 & 0.81 $\pm$ 0.06 & 0.85 $\pm$ 0.02 & 0.79 $\pm$ 0.09 & 0.78 $\pm$ 0.02 \\
S-BERT XLM-R & 0.70 $\pm$ 0.10 & 0.73 $\pm$ 0.05 & 0.69 $\pm$ 0.11 & 0.65 $\pm$ 0.10 & 0.78 $\pm$ 0.10 & 0.85 $\pm$ 0.07 & 0.76 $\pm$ 0.10 & 0.70 $\pm$ 0.08 \\
Hybrid XLM-R (k=64) & \textbf{0.79} $\pm$ 0.07 & 0.82 $\pm$ 0.04 & \textbf{0.79} $\pm$ 0.07 & \textbf{0.75} $\pm$ 0.08 & \textbf{0.89} $\pm$ 0.05 & 0.92 $\pm$ 0.04 & \textbf{0.88} $\pm$ 0.05 & \textbf{0.87} $\pm$ 0.05 \\

% NMT + USE & 0.73 & 0.78 & 0.77 & 0.57 & 0.77 & 0.78 & 0.76 & 0.78 \\\hline
% mUSE & 0.71 & \textbf{0.87} & 0.57 & 0.72 & 0.68 & \textbf{0.94} & 0.66 & 0.34 \\
% LASER & 0.73 & 0.69 & 0.82 & 0.63 & 0.46 & 0.54 & 0.64 & 0.18 \\
% S-BERT & 0.72 & 0.72 & 0.72 & 0.71 & 0.81 & 0.85 & 0.79 & 0.78 \\
% S-BERT XLM-R & 0.70 & 0.73 & 0.69 & 0.65 & 0.78 & 0.85 & 0.76 & 0.70 \\
% Hybrid XLM-R (k=64) & \textbf{0.79} & 0.82 & \textbf{0.79} & \textbf{0.75} & \textbf{0.89} & 0.92 & \textbf{0.88} & \textbf{0.87} \\
\bottomrule
\end{tabular}
\end{small}
\caption{XX $\rightarrow$ EN Accuracies: The average accuracies obtained for each method on mapping from queries in a given language to English. Only a subset of the MQKA langauge results are shown: 5 of the languages NMT + USE performs the best, and 5 which it is least performant.}
\end{table*}

==> tables/xxen_xquad.tex <==

\begin{table*}[]
\centering
\begin{tabular}{lccccccccccc}
\toprule
 & \multicolumn{10}{c}{XX $\rightarrow$ EN} \\
\cmidrule{2-12}
 & \multicolumn{1}{|l|}{avg} & ar & de & el & es & hi & ru & th & tr & vi & zh\\
\midrule
NMT USE-L & \multicolumn{1}{|l|}{0.89} & 0.86 & 0.97 & 0.95 & 0.98 & 0.91 & 0.93 & 0.84 & 0.93 & 0.88 & 0.66 \\\hline
LASER & \multicolumn{1}{|l|}{0.64} & 0.79 & 0.53 & 0.08 & 0.94 & 0.51 & 0.83 & 0.47 & 0.85 & 0.83 & 0.56 \\
MUSE-L & \multicolumn{1}{|l|}{0.73} & 0.95 & 0.98 & 0.13 & 0.99 & 0.08 & 0.97 & 0.96 & 0.97 & 0.26 & 0.96 \\
SBERT XLM-R & \multicolumn{1}{|l|}{0.45} & 0.33 & 0.64 & 0.47 & 0.67 & 0.33 & 0.45 & 0.36 & 0.41 & 0.48 & 0.31 \\
XLM-R & \multicolumn{1}{|l|}{0.84} & 0.81 & 0.83 & 0.89 & 0.89 & 0.90 & 0.80 & 0.80 & 0.85 & 0.84 & 0.79 \\
XLM-R (75, 25) & \multicolumn{1}{|l|}{0.96} & 0.94 & 0.95 & 0.98 & 0.98 & 0.96 & 0.95 & 0.96 & 0.96 & 0.95 & 0.94 \\
XLM-R (50, 50) & \multicolumn{1}{|l|}{0.95} & 0.94 & 0.94 & 0.97 & 0.97 & 0.96 & 0.92 & 0.96 & 0.95 & 0.94 & 0.93 \\
BERT (75, 25) & \multicolumn{1}{|l|}{0.63} & 0.57 & 0.86 & 0.63 & 0.90 & 0.50 & 0.79 & 0.13 & 0.56 & 0.70 & 0.64 \\
SBERT XLM-R (Distil) & \multicolumn{1}{|l|}{0.86} & 0.76 & 0.93 & 0.89 & 0.94 & 0.84 & 0.89 & 0.78 & 0.84 & 0.90 & 0.84 \\
SBERT XLM-R (75, 25) & \multicolumn{1}{|l|}{0.89} & 0.81 & 0.95 & 0.90 & 0.96 & 0.88 & 0.92 & 0.78 & 0.90 & 0.92 & 0.88 \\
Hybrid XLM-R (k=4) & \multicolumn{1}{|l|}{0.95} & 0.88 & 0.98 & 0.95 & 0.98 & 0.94 & 0.96 & 0.87 & 0.96 & 0.96 & 0.93 \\
Hybrid XLM-R (k=8) & \multicolumn{1}{|l|}{0.96} & 0.90 & 0.98 & 0.96 & 0.98 & 0.95 & 0.96 & 0.90 & 0.96 & 0.96 & 0.94 \\
Hybrid XLM-R (k=16) & \multicolumn{1}{|l|}{0.96} & 0.92 & 0.98 & 0.97 & 0.98 & 0.96 & 0.97 & 0.92 & 0.97 & 0.96 & 0.95 \\
Hybrid XLM-R (k=32) & \multicolumn{1}{|l|}{\textbf{0.97}} & 0.94 & 0.98 & 0.98 & 0.98 & 0.96 & 0.97 & 0.93 & 0.98 & 0.97 & 0.95 \\
Hybrid XLM-R (k=64) & \multicolumn{1}{|l|}{\textbf{0.97}} & 0.95 & 0.98 & 0.98 & 0.98 & 0.97 & 0.97 & 0.94 & 0.98 & 0.97 & 0.95 \\
Hybrid XLM-R (k=128 & \multicolumn{1}{|l|}{\textbf{0.97}} & 0.95 & 0.98 & 0.98 & 0.99 & 0.97 & 0.97 & 0.95 & 0.98 & 0.97 & 0.95 \\
Hybrid XLM-R (k=256) & \multicolumn{1}{|l|}{\textbf{0.97}} & 0.95 & 0.98 & 0.98 & 0.99 & 0.97 & 0.97 & 0.95 & 0.98 & 0.97 & 0.95 \\
Hybrid XLM-R (k=512) & \multicolumn{1}{|l|}{\textbf{0.97}} & 0.95 & 0.98 & 0.98 & 0.99 & 0.97 & 0.97 & 0.96 & 0.98 & 0.97 & 0.95 \\
Hybrid XLM-R (k=1024) & \multicolumn{1}{|l|}{\textbf{0.97}} & 0.95 & 0.98 & 0.98 & 0.99 & 0.97 & 0.97 & 0.96 & 0.98 & 0.97 & 0.95 \\
\bottomrule
\end{tabular}
\caption{XQuAD XX $\rightarrow$ EN Accuracies}
\end{table*}

==> tables/xxen_xquad_distractor.tex <==

\begin{table*}[htbp]
\centering
\begin{tabular}{lccccccccccc}
\toprule
 & \multicolumn{10}{c}{XQuAD + SQuAD} \\
\cmidrule{2-12}
 & \multicolumn{1}{|c|}{avg} & ar & de & el & es & hi & ru & th & tr & vi & zh \\
\midrule
NMT + USE & \multicolumn{1}{|c|}{0.77} & 0.71 & 0.91 & 0.86 & 0.95 & 0.79 & 0.85 & 0.67 & 0.82 & 0.74 & 0.41 \\
mUSE & \multicolumn{1}{|c|}{0.68} & \textbf{0.87} & \textbf{0.96} & 0.07 & \textbf{0.98} & 0.03 & \textbf{0.93} & \textbf{0.91} & \textbf{0.94} & 0.17 & \textbf{0.90} \\
LASER & \multicolumn{1}{|c|}{0.46} & 0.61 & 0.33 & 0.03 & 0.86 & 0.28 & 0.70 & 0.24 & 0.65 & 0.64 & 0.29 \\
S-BERT & \multicolumn{1}{|c|}{0.81} & 0.66 & 0.85 & 0.81 & 0.87 & 0.77 & 0.85 & 0.76 & 0.81 & 0.89 & 0.82 \\
S-BERT XLM-R & \multicolumn{1}{|c|}{0.78} & 0.62 & 0.90 & 0.79 & 0.93 & 0.72 & 0.82 & 0.60 & 0.81 & 0.85 & 0.75 \\
Hybrid XLM-R (k=4) & \multicolumn{1}{|c|}{0.83} & 0.70 & 0.94 & 0.84 & 0.94 & 0.79 & 0.87 & 0.68 & 0.87 & 0.89 & 0.81 \\
Hybrid XLM-R (k=8) & \multicolumn{1}{|c|}{0.85} & 0.73 & 0.94 & 0.87 & 0.94 & 0.81 & 0.89 & 0.71 & 0.88 & 0.91 & 0.83 \\
Hybrid XLM-R (k=16) & \multicolumn{1}{|c|}{0.87} & 0.76 & 0.95 & 0.89 & 0.96 & 0.84 & 0.89 & 0.75 & 0.89 & 0.91 & 0.85 \\
Hybrid XLM-R (k=32) & \multicolumn{1}{|c|}{0.89} & 0.79 & 0.95 & 0.90 & 0.96 & 0.87 & 0.91 & 0.77 & 0.91 & \textbf{0.92} & 0.86 \\
Hybrid XLM-R (k=64) & \multicolumn{1}{|c|}{0.89} & 0.81 & 0.95 & \textbf{0.91} & 0.96 & \textbf{0.89} & 0.91 & 0.80 & 0.91 & 0.91 & 0.87 \\

\bottomrule

\end{tabular}
\caption{XX $\rightarrow$ EN Accuracies: TODO}
\end{table*}


==> tables/xxenxx_partial.tex <==

\begin{table*}[htbp]
\centerline{
\begin{tiny}
\begin{tabular}{lccccccccccc}
\toprule
 & \multicolumn{10}{c}{XQuAD + SQuAD (NMT)} \\
\cmidrule{2-12}
 & \multicolumn{1}{|c|}{avg} & es & de & vi & tr & el & ar & hi & ru & zh & th \\
 \midrule
 
NMT + USE & \multicolumn{1}{|c|}{0.39 \pm 0.15 (0.24 \pm 0.12)} & 0.68 (0.48) & 0.56 (0.43) & 0.39 (0.23) & 0.31 (0.17) & 0.42 (0.28) & 0.33 (0.19) & 0.46 (0.25) & 0.35 (0.20) & 0.18 (0.14) & 0.19 (0.07) \\\midrule
mUSE & \multicolumn{1}{|c|}{0.32 \pm 0.21 (0.21 \pm 0.16)} & \textbf{0.70 (0.50)} & \textbf{0.58 (0.45)} & 0.04 (0.03) & \textbf{0.33 (0.19)} & \textbf{0.47 (0.31)} & 0.02 (0.01) & 0.12 (0.07) & \textbf{0.41 (0.23)} & \textbf{0.23 (0.18)} & \textbf{0.34 (0.14)} \\
LASER & \multicolumn{1}{|c|}{0.24 \pm 0.17 (0.15 \pm 0.12)} & 0.62 (0.43) & 0.23 (0.18) & 0.02 (0.01) & 0.24 (0.14) & 0.33 (0.22) & 0.11 (0.06) & 0.39 (0.21) & 0.30 (0.17) & 0.06 (0.05) & 0.13 (0.05) \\
S-BERT & \multicolumn{1}{|c|}{0.39 \pm 0.13 (0.24 \pm 0.11)} & 0.64 (0.46) & 0.53 (0.41) & 0.37 (0.22) & 0.30 (0.17) & 0.42 (0.28) & 0.31 (0.17) & 0.53 (0.29) & 0.31 (0.17) & 0.19 (0.14) & 0.31 (0.13) \\
S-BERT XLM-R & \multicolumn{1}{|c|}{0.38 \pm 0.15 (0.24 \pm 0.12)} & 0.67 (0.47) & 0.55 (0.43) & 0.35 (0.20) & 0.29 (0.16) & 0.42 (0.27) & 0.28 (0.15) & 0.51 (0.27) & 0.29 (0.16) & 0.15 (0.12) & 0.28 (0.12) \\
Hybrid XLM-R (k=64) & \multicolumn{1}{|c|}{0.43 \pm 0.14 (0.26 \pm 0.11)} & 0.69 (0.49) & \textbf{0.58 (0.45)} & \textbf{0.40 (0.23)} & 0.32 (0.18) & 0.46 (0.30) & \textbf{0.35 (0.20)} & \textbf{0.54 (0.29)} & 0.38 (0.21) & 0.20 (0.15) & 0.33 (0.13) \\\midrule


% Hybrid XLM-R (k=32) & \multicolumn{1}{|c|}{0.42 \pm 0.14 (0.26 \pm 0.12)} & 0.69 (0.49) & \textbf{0.58 (0.45)} & \textbf{0.40 (0.23)} & 0.32 (0.18) & 0.45 (0.30) & 0.34 (0.19) & \textbf{0.54 (0.29)} & 0.37 (0.21) & 0.19 (0.15) & 0.32 (0.13) \\
% Hybrid XLM-R (k=16) & \multicolumn{1}{|c|}{0.42 \pm 0.14 (0.26 \pm 0.12)} & 0.69 (0.49) & \textbf{0.58 (0.44)} & \textbf{0.40 (0.23)} & 0.31 (0.17) & 0.45 (0.30) & 0.33 (0.19) & \textbf{0.54 (0.29)} & 0.36 (0.19) & 0.18 (0.14) & 0.32 (0.13) \\
% Hybrid XLM-R (k=8) & \multicolumn{1}{|c|}{0.41 \pm 0.14 (0.25 \pm 0.12)} & 0.68 (0.49) & 0.57 (0.44) & 0.39 (0.23) & 0.31 (0.18) & 0.44 (0.29) & 0.32 (0.18) & 0.53 (0.29) & 0.34 (0.19) & 0.18 (0.13) & 0.31 (0.13) \\
% Hybrid XLM-R (k=4) & \multicolumn{1}{|c|}{0.40 \pm 0.14 (0.25 \pm 0.12)} & 0.68 (0.49) & 0.57 (0.44) & 0.38 (0.22) & 0.31 (0.17) & 0.44 (0.29) & 0.31 (0.18) & 0.53 (0.29) & 0.33 (0.18) & 0.17 (0.13) & 0.31 (0.13) \\
 
 
% NMT + USE & \multicolumn{1}{|c|}{0.39 (0.24)} & 0.68 (0.48) & 0.56 (0.43) & 0.46 (0.25) & 0.42 (0.28) & 0.39 (0.23) & 0.35 (0.20) & 0.33 (0.19) & 0.31 (0.17) & 0.19 (0.07) & 0.18 (0.14) \\\midrule
% mUSE & \multicolumn{1}{|c|}{0.32 (0.21)} & \textbf{0.70 (0.50)} & \textbf{0.58 (0.45)} & 0.12 (0.07) & \textbf{0.47 (0.31)} & 0.04 (0.03) & \textbf{0.41 (0.23)} & 0.02 (0.01) & \textbf{0.33 (0.19)} & \textbf{0.34 (0.14)} & \textbf{0.23 (0.18)} \\
% LASER & \multicolumn{1}{|c|}{0.24 (0.15)} & 0.62 (0.43) & 0.23 (0.18) & 0.39 (0.21) & 0.33 (0.22) & 0.02 (0.01) & 0.30 (0.17) & 0.11 (0.06) & 0.24 (0.14) & 0.13 (0.05) & 0.06 (0.05) \\
% S-BERT & \multicolumn{1}{|c|}{0.39 (0.24)} & 0.64 (0.46) & 0.53 (0.41) & 0.53 (0.29) & 0.42 (0.28) & 0.37 (0.22) & 0.31 (0.17) & 0.31 (0.17) & 0.30 (0.17) & 0.31 (0.13) & 0.19 (0.14) \\
% S-BERT XLM-R & \multicolumn{1}{|c|}{0.38 (0.24)} & 0.67 (0.47) & 0.55 (0.43) & 0.51 (0.27) & 0.42 (0.27) & 0.35 (0.20) & 0.29 (0.16) & 0.28 (0.15) & 0.29 (0.16) & 0.28 (0.12) & 0.15 (0.12) \\
% Hybrid XLM-R (k=64) & \multicolumn{1}{|c|}{\textbf{0.43 (0.26)}} & 0.69 (0.49) & \textbf{0.58 (0.45)} & \textbf{0.54 (0.29)} & 0.46 (0.30) & \textbf{\textbf{0.40 (0.23)}} & 0.38 (0.21) & \textbf{0.35 (0.20)} & 0.32 (0.18) & 0.33 (0.13) & 0.20 (0.15) \\\midrule




\textit{Perfect XX $\rightarrow$ EN} & \multicolumn{1}{|c|}{0.47 \pm 0.13 (0.29 \pm 0.11)} & 0.87 (0.79) & 0.90 (0.85) & 0.89 (0.83) & 0.86 (0.77) & 0.90 (0.85) & 0.75 (0.65) & 0.75 (0.56) & 0.51 (0.45) & 0.65 (0.58) & 0.33 (0.32) \\

% xquad: 0.29 \pm 0.11 (0.47 \pm 0.13)
% mkqa: 0.76 \pm 0.18 (0.69 \pm 0.17)

\midrule
 & \multicolumn{10}{c}{MKQA + Natural Questions (WikiData)} \\
\cmidrule{2-12}
%  & \multicolumn{1}{|c|}{avg} & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ \\
% \midrule
% NMT + USE & \multicolumn{1}{|c|}{\_\_} & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ \\\hline
% \_\_ & \multicolumn{1}{|c|}{\_\_} & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ \\
% \_\_ & \multicolumn{1}{|c|}{\_\_} & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ \\
% \_\_ & \multicolumn{1}{|c|}{\_\_} & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ \\\hline

 & \multicolumn{1}{|c|}{avg} & da & nl & fr & pt & de & ar & ja & ko & km & $zh_{tw}$ \\
\midrule


NMT + USE & \multicolumn{1}{|c|}{0.69 \pm 0.16 (0.66 \pm 0.16)} & \textbf{0.86 (0.83)} & 0.85 (0.82) & 0.84 (0.81) & 0.83 (0.80) & 0.84 (0.81) & 0.60 (0.58) & 0.60 (0.54) & 0.47 (0.46) & 0.45 (0.38) & 0.35 (0.32) \\\midrule
mUSE & \multicolumn{1}{|c|}{0.66 \pm 0.19 (0.63 \pm 0.18)} & 0.50 (0.49) & 0.89 (0.85) & \textbf{0.88 (0.84)} & \textbf{0.89 (0.86)} & \textbf{0.87 (0.84)} & 0.69 (0.66) & \textbf{0.75 (0.69)} & \textbf{0.63 (0.61)} & 0.35 (0.32) & \textbf{0.56 (0.50)} \\
LASER & \multicolumn{1}{|c|}{0.68 \pm 0.15 (0.65 \pm 0.15)} & 0.85 (0.82) & \textbf{0.90 (0.87)} & 0.75 (0.73) & 0.81 (0.78) & 0.51 (0.50) & \textbf{0.70 (0.68)} & 0.39 (0.36) & 0.59 (0.57) & 0.38 (0.36) & 0.46 (0.42) \\
S-BERT & \multicolumn{1}{|c|}{0.67 \pm 0.08 (0.63 \pm 0.08)} & 0.81 (0.78) & 0.76 (0.73) & 0.71 (0.68) & 0.63 (0.60) & 0.72 (0.69) & 0.51 (0.49) & 0.68 (0.62) & 0.62 (0.60) & 0.55 (0.47) & 0.54 (0.49) \\
S-BERT XLM-R & \multicolumn{1}{|c|}{0.65 \pm 0.11 (0.62 \pm 0.11)} & 0.82 (0.78) & 0.81 (0.78) & 0.75 (0.72) & 0.73 (0.70) & 0.77 (0.74) & 0.46 (0.45) & 0.63 (0.56) & 0.54 (0.52) & 0.49 (0.41) & 0.48 (0.44) \\
Hybrid XLM-R (k=64) & \multicolumn{1}{|c|}{0.73 \pm 0.09 (0.70 \pm 0.10)} & 0.85 (0.82) & 0.85 (0.82) & 0.82 (0.79) & 0.82 (0.78) & 0.83 (0.80) & 0.59 (0.57) & 0.72 (0.66) & 0.61 (0.59) & \textbf{0.59 (0.51)} & 0.55 (0.49) \\\midrule
% Hybrid XLM-R (k=32) & \multicolumn{1}{|c|}{0.73 \pm 0.09 (0.69 \pm 0.10)} & 0.85 (0.81) & 0.85 (0.82) & 0.82 (0.79) & 0.81 (0.78) & 0.83 (0.79) & 0.58 (0.56) & 0.71 (0.65) & 0.61 (0.59) & 0.58 (0.50) & 0.55 (0.49) \\
% Hybrid XLM-R (k=16) & \multicolumn{1}{|c|}{0.72 \pm 0.10 (0.69 \pm 0.10)} & 0.85 (0.81) & 0.85 (0.81) & 0.81 (0.78) & 0.80 (0.77) & 0.82 (0.79) & 0.57 (0.55) & 0.70 (0.65) & 0.61 (0.59) & 0.57 (0.50) & 0.54 (0.49) \\
% Hybrid XLM-R (k=8) & \multicolumn{1}{|c|}{0.72 \pm 0.10 (0.68 \pm 0.10)} & 0.85 (0.81) & 0.84 (0.81) & 0.81 (0.78) & 0.80 (0.77) & 0.82 (0.79) & 0.56 (0.54) & 0.69 (0.63) & 0.61 (0.59) & 0.56 (0.49) & 0.54 (0.49) \\
% Hybrid XLM-R (k=4) & \multicolumn{1}{|c|}{0.71 \pm 0.10 (0.68 \pm 0.10)} & 0.85 (0.81) & 0.84 (0.81) & 0.80 (0.77) & 0.79 (0.76) & 0.81 (0.78) & 0.55 (0.53) & 0.68 (0.63) & 0.60 (0.58) & 0.54 (0.48) & 0.53 (0.49) \\




% NMT + USE & \multicolumn{1}{|c|}{0.69 (0.66)} & \textbf{0.86 (0.83)} & 0.85 (0.82) & 0.84 (0.81) & 0.83 (0.80) & 0.84 (0.81) & 0.60 (0.58) & 0.60 (0.54) & 0.47 (0.46) & 0.45 (0.38) & 0.35 (0.32) \\\midrule
% mUSE & \multicolumn{1}{|c|}{0.66 (0.63)} & 0.50 (0.49) & 0.89 (0.85) & \textbf{0.88 (0.84)} & \textbf{0.89 (0.86)} & \textbf{0.87 (0.84)} & 0.69 (0.66) & \textbf{0.75 (0.69)} & \textbf{0.63 (0.61)} & 0.35 (0.32) & \textbf{0.56 (0.50)} \\
% LASER & \multicolumn{1}{|c|}{0.68 (0.65)} & 0.85 (0.82) & \textbf{0.90 (0.87)} & 0.75 (0.73) & 0.81 (0.78) & 0.51 (0.50) & \textbf{0.70 (0.68)} & 0.39 (0.36) & 0.59 (0.57) & 0.38 (0.36) & 0.46 (0.42) \\
% S-BERT & \multicolumn{1}{|c|}{0.67 (0.63)} & 0.81 (0.78) & 0.76 (0.73) & 0.71 (0.68) & 0.63 (0.60) & 0.72 (0.69) & 0.51 (0.49) & 0.68 (0.62) & 0.62 (0.60) & 0.55 (0.47) & 0.54 (0.49) \\
% S-BERT XLM-R & \multicolumn{1}{|c|}{0.65 (0.62)} & 0.82 (0.78) & 0.81 (0.78) & 0.75 (0.72) & 0.73 (0.70) & 0.77 (0.74) & 0.46 (0.45) & 0.63 (0.56) & 0.54 (0.52) & 0.49 (0.41) & 0.48 (0.44) \\
% Hybrid XLM-R (k=64) & \multicolumn{1}{|c|}{\textbf{0.73 (0.70)}} & 0.85 (0.82) & 0.85 (0.82) & 0.82 (0.79) & 0.82 (0.78) & 0.83 (0.80) & 0.59 (0.57) & 0.72 (0.66) & 0.61 (0.59) & \textbf{0.59 (0.51)} & 0.55 (0.49) \\\midrule

%  & \multicolumn{1}{|c|}{avg} & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ \\
% \midrule
% NMT + USE & \multicolumn{1}{|c|}{\_\_} & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ \\\hline
% \_\_ & \multicolumn{1}{|c|}{\_\_} & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ \\
% \_\_ & \multicolumn{1}{|c|}{\_\_} & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ \\
% \_\_ & \multicolumn{1}{|c|}{\_\_} & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ \\\hline
\textit{Perfect XX $\rightarrow$ EN} & \multicolumn{1}{|c|}{0.76 \pm 0.18 (0.69 \pm 0.17)} & 0.87 (0.79) & 0.90 (0.85) & 0.89 (0.83) & 0.86 (0.77) & 0.90 (0.85) & 0.75 (0.65) & 0.75 (0.56) & 0.51 (0.45) & 0.65 (0.58) & 0.33 (0.32) \\

% \bottomrule
% \toprule
%  & \multicolumn{10}{c}{MKQA} \\
% \cmidrule{2-13}
%  & \multicolumn{1}{|c}{avg} & \multicolumn{1}{c|}{std} & ar & da & de & es & fi & fr & he & hu & it & ja\\
% \midrule
% NMT USE-L & \multicolumn{1}{|l}{0.82} & \multicolumn{1}{l|}{0.093} & 0.80 & \textbf{0.95} & 0.94 & 0.93 & 0.86 & 0.94 & 0.85 & 0.89 & 0.93 & 0.75 \\\hline
% LASER & \multicolumn{1}{|l}{0.79} & \multicolumn{1}{l|}{0.260} & \textbf{0.90} & 0.93 & 0.58 & 0.87 & 0.89 & 0.86 & \textbf{0.92} & 0.78 & 0.87 & 0.51 \\
% MUSE-L & \multicolumn{1}{|l}{0.51} & \multicolumn{1}{l|}{0.395} & 0.89 & 0.65 & \textbf{0.96} & \textbf{0.97} & 0.48 & \textbf{0.96} & 0.32 & 0.51 & \textbf{0.96} & \textbf{0.89} \\
% XLM-R & \multicolumn{1}{|l}{\textbf{0.91}} & \multicolumn{1}{l|}{\textbf{0.014}} & 0.83 & \textbf{0.95} & 0.93 & \textbf{0.94} & \textbf{0.91} & 0.92 & 0.89 & \textbf{0.90} & 0.92 & 0.88 \\
% SBERT XLM-R & \multicolumn{1}{|l}{0.85} & \multicolumn{1}{l|}{0.057} & 0.63 & 0.92 & 0.88 & 0.88 & 0.76 & 0.87 & 0.73 & 0.78 & 0.83 & 0.77 \\
% Hybrid XLM-R & \multicolumn{1}{|l}{\textbf{0.91}} & \multicolumn{1}{l|}{\textbf{0.014}} & 0.78 & \textbf{0.95} & 0.93 & 0.93 & 0.88 & 0.93 & 0.87 & 0.88 & 0.91 & 0.87 \\
\bottomrule

\end{tabular}
\end{tiny}}
\caption{End-To-End F1 and EM: The average F1 (EM) scores obtained for each method when mapping from queries in a given language to English then back to the original language. We use a Many-to-Many NMT to generate the language in the original langauge for XQuAD, and WikiData translation for MKQA. For reference, \textit{Perfect XX $\rightarrow$ EN} shows the results obtained when using the ground truth English answer in back translation. Only a subset of the MQKA langauge results are shown: 5 of the languages NMT + USE performs the best, and 5 which it's least performant. Averages are across all languages in the dataset.}
\end{table*}


%  & \multicolumn{1}{|c|}{avg} & es & de & vi & tr & el & ar & hi & ru & zh & th \\
% \midrule
% NMT + USE & \multicolumn{1}{|c|}{0.39 (0.24)} & 0.68 (0.48) & 0.56 (0.43) & 0.46 (0.25) & 0.42 (0.28) & 0.39 (0.23) & 0.35 (0.20) & 0.33 (0.19) & 0.31 (0.17) & 0.19 (0.07) & 0.18 (0.14) \\
% mUSE & \multicolumn{1}{|c|}{0.32 (0.21)} & \textbf{0.70 (0.50)} & \textbf{0.58 (0.45)} & 0.12 (0.07) & \textbf{0.47 (0.31)} & 0.04 (0.03) & \textbf{0.41 (0.23)} & 0.02 (0.01) & \textbf{0.33 (0.19)} & \textbf{0.34 (0.14)} & \textbf{0.23 (0.18)} \\
% LASER & \multicolumn{1}{|c|}{0.24 (0.15)} & 0.62 (0.43) & 0.23 (0.18) & 0.39 (0.21) & 0.33 (0.22) & 0.02 (0.01) & 0.30 (0.17) & 0.11 (0.06) & 0.24 (0.14) & 0.13 (0.05) & 0.06 (0.05) \\
% S-BERT & \multicolumn{1}{|c|}{0.39 (0.24)} & 0.64 (0.46) & 0.53 (0.41) & 0.53 (0.29) & 0.42 (0.28) & 0.37 (0.22) & 0.31 (0.17) & 0.31 (0.17) & 0.30 (0.17) & 0.31 (0.13) & 0.19 (0.14) \\
% S-BERT XLM-R & \multicolumn{1}{|c|}{0.38 (0.24)} & 0.67 (0.47) & 0.55 (0.43) & 0.51 (0.27) & 0.42 (0.27) & 0.35 (0.20) & 0.29 (0.16) & 0.28 (0.15) & 0.29 (0.16) & 0.28 (0.12) & 0.15 (0.12) \\
% Hybrid XLM-R (k=64) & \multicolumn{1}{|c|}{0.43 (0.26)} & 0.69 (0.49) & \textbf{0.58 (0.45)} & \textbf{0.54 (0.29)} & 0.46 (0.30) & \textbf{0.40 (0.23)} & 0.38 (0.21) & \textbf{0.35 (0.20)} & 0.32 (0.18) & 0.33 (0.13) & 0.20 (0.15) \\
% Hybrid XLM-R (k=32) & \multicolumn{1}{|c|}{0.42 (0.26)} & 0.69 (0.49) & \textbf{0.58 (0.45)} & \textbf{0.54 (0.29)} & 0.45 (0.30) & \textbf{0.40 (0.23)} & 0.37 (0.21) & 0.34 (0.19) & 0.32 (0.18) & 0.32 (0.13) & 0.19 (0.15) \\
% Hybrid XLM-R (k=16) & \multicolumn{1}{|c|}{0.42 (0.26)} & 0.69 (0.49) & \textbf{0.58 (0.44)} & \textbf{0.54 (0.29)} & 0.45 (0.30) & \textbf{0.40 (0.23)} & 0.36 (0.19) & 0.33 (0.19) & 0.31 (0.17) & 0.32 (0.13) & 0.18 (0.14) \\
% Hybrid XLM-R (k=8) & \multicolumn{1}{|c|}{0.41 (0.25)} & 0.68 (0.49) & 0.57 (0.44) & 0.53 (0.29) & 0.44 (0.29) & 0.39 (0.23) & 0.34 (0.19) & 0.32 (0.18) & 0.31 (0.18) & 0.31 (0.13) & 0.18 (0.13) \\
% Hybrid XLM-R (k=4) & \multicolumn{1}{|c|}{0.40 (0.25)} & 0.68 (0.49) & 0.57 (0.44) & 0.53 (0.29) & 0.44 (0.29) & 0.38 (0.22) & 0.33 (0.18) & 0.31 (0.18) & 0.31 (0.17) & 0.31 (0.13) & 0.17 (0.13) \\


%  & XQuAD (NMT) & MKQA (WikiData) \\
% \midrule
% el&0.26 (0.45)&-(-)\\
% hi&0.23 (0.40)&-(-)\\
% ru&0.20 (0.35)&0.71 (0.65)\\
% de&0.47 (0.61)&0.90 (0.85)\\
% ar&0.26 (0.46)&0.75 (0.65)\\
% zh&0.15 (0.37)&-(-)\\
% th&0.19 (0.25)&0.73 (0.61)\\
% es&0.51 (0.71)&0.90 (0.84)\\
% tr&0.32 (0.50)&0.87 (0.79)\\
% vi&0.31 (0.58)&0.86 (0.77)\\
% zh-tw&-(-)&0.33 (0.32)\\
% ko&-(-)&0.51 (0.45)\\
% no&-(-)&0.88 (0.82)\\
% zh-hk&-(-)&0.34 (0.32)\\
% pl&-(-)&0.84 (0.76)\\
% hu&-(-)&0.85 (0.77)\\
% ja&-(-)&0.75 (0.56)\\
% he&-(-)&0.75 (0.64)\\
% it&-(-)&0.89 (0.84)\\
% nl&-(-)&0.90 (0.85)\\
% fi&-(-)&0.84 (0.77)\\
% ms&-(-)&0.89 (0.83)\\
% zh-cn&-(-)&0.33 (0.32)\\
% km&-(-)&0.65 (0.58)\\
% pt&-(-)&0.86 (0.77)\\
% fr&-(-)&0.89 (0.83)\\
% da&-(-)&0.87 (0.79)\\
% sv&-(-)&0.86 (0.78)\\
% \bottomrule

% xquad: 0.29 (0.47)
% mkqa: 0.76 (0.69)

% 0.87 (0.79) & 0.90 (0.85) & 0.89 (0.83) & 0.86 (0.77) & 0.90 (0.85) & 0.75 (0.65) & 0.75 (0.56) & 0.51 (0.45) & 0.65 (0.58) & 0.33 (0.32)

==> tables/xxenxx_partial_groups.tex <==

\begin{table*}[htbp]
\centerline{
\begin{small}
\begin{tabular}{lcccc}
\toprule
 & \multicolumn{4}{c}{XQuAD + SQuAD (NMT)} \\
\cmidrule{2-5}
 & \multicolumn{1}{|c|}{avg} & High & Medium & Low \\
 \midrule

NMT + USE & \multicolumn{1}{|c|}{0.39 $\pm$ 0.15 (0.24 $\pm$ 0.12)} & 0.43 $\pm$ 0.19 (0.29 $\pm$ 0.17) & 0.41 $\pm$ 0.04 (0.25 $\pm$ 0.03) & 0.30 $\pm$ 0.09 (0.19 $\pm$ 0.04) \\\hline
mUSE & \multicolumn{1}{|c|}{0.32 $\pm$ 0.21 (0.21 $\pm$ 0.16)} & \textbf{0.49} $\pm$ 0.16 (0.32 $\pm$ 0.16) & 0.33 $\pm$ 0.15 (0.20 $\pm$ 0.10) & 0.10 $\pm$ 0.10 (0.07 $\pm$ 0.08) \\
LASER & \multicolumn{1}{|c|}{0.24 $\pm$ 0.17 (0.15 $\pm$ 0.12)} & 0.30 $\pm$ 0.19 (0.20 $\pm$ 0.14) & 0.34 $\pm$ 0.04 (0.20 $\pm$ 0.02) & 0.06 $\pm$ 0.04 (0.04 $\pm$ 0.02) \\
S-BERT & \multicolumn{1}{|c|}{0.39 $\pm$ 0.13 (0.24 $\pm$ 0.11)} & 0.44 $\pm$ 0.15 (0.29 $\pm$ 0.14) & 0.42 $\pm$ 0.09 (0.25 $\pm$ 0.05) & 0.29 $\pm$ 0.08 (0.18 $\pm$ 0.03) \\
S-BERT XLM-R & \multicolumn{1}{|c|}{0.38 $\pm$ 0.15 (0.24 $\pm$ 0.12)} & 0.45 $\pm$ 0.17 (0.30 $\pm$ 0.16) & 0.41 $\pm$ 0.09 (0.24 $\pm$ 0.05) & 0.26 $\pm$ 0.08 (0.16 $\pm$ 0.03) \\
Hybrid XLM-R (k=64) & \multicolumn{1}{|c|}{\textbf{0.43} $\pm$ 0.14 (0.26 $\pm$ 0.11)} & 0.48 $\pm$ 0.16 (0.31 $\pm$ 0.16) & \textbf{0.46} $\pm$ 0.07 (0.27 $\pm$ 0.04) & \textbf{0.32} $\pm$ 0.09 (0.19 $\pm$ 0.03) \\
% Hybrid XLM-R (k=32) & \multicolumn{1}{|c|}{0.42 $\pm$ 0.14 (0.26 $\pm$ 0.12)} & 0.48 $\pm$ 0.16 (0.31 $\pm$ 0.16) & 0.46 $\pm$ 0.07 (0.27 $\pm$ 0.04) & 0.31 $\pm$ 0.09 (0.19 $\pm$ 0.04) \\
% Hybrid XLM-R (k=16) & \multicolumn{1}{|c|}{0.42 $\pm$ 0.14 (0.26 $\pm$ 0.12)} & 0.47 $\pm$ 0.16 (0.31 $\pm$ 0.16) & 0.45 $\pm$ 0.08 (0.26 $\pm$ 0.05) & 0.30 $\pm$ 0.09 (0.19 $\pm$ 0.04) \\
% Hybrid XLM-R (k=8) & \multicolumn{1}{|c|}{0.41 $\pm$ 0.14 (0.25 $\pm$ 0.12)} & 0.47 $\pm$ 0.16 (0.31 $\pm$ 0.16) & 0.44 $\pm$ 0.08 (0.25 $\pm$ 0.05) & 0.30 $\pm$ 0.09 (0.18 $\pm$ 0.04) \\
% Hybrid XLM-R (k=4) & \multicolumn{1}{|c|}{0.40 $\pm$ 0.14 (0.25 $\pm$ 0.12)} & 0.47 $\pm$ 0.16 (0.31 $\pm$ 0.16) & 0.43 $\pm$ 0.08 (0.25 $\pm$ 0.05) & 0.29 $\pm$ 0.09 (0.17 $\pm$ 0.04) \\
\midrule
\textit{Perfect XX $\rightarrow$ EN} & \multicolumn{1}{|c|}{0.76 $\pm$ 0.18 (0.69 $\pm$ 0.17)} & 0.51 $\pm$ 0.16 (0.33 $\pm$ 0.16) & 0.51 $\pm$ 0.05 (0.30 $\pm$ 0.03) & 0.36 $\pm$ 0.08 (0.23 $\pm$ 0.03) \\

 
% NMT + USE & \multicolumn{1}{|c|}{0.39 \pm 0.15 (0.24 \pm 0.12)} & 0.68 (0.48) & 0.56 (0.43) & 0.39 (0.23) & 0.31 (0.17) & 0.42 (0.28) & 0.33 (0.19) & 0.46 (0.25) & 0.35 (0.20) & 0.18 (0.14) & 0.19 (0.07) \\\midrule
% mUSE & \multicolumn{1}{|c|}{0.32 \pm 0.21 (0.21 \pm 0.16)} & \textbf{0.70 (0.50)} & \textbf{0.58 (0.45)} & 0.04 (0.03) & \textbf{0.33 (0.19)} & \textbf{0.47 (0.31)} & 0.02 (0.01) & 0.12 (0.07) & \textbf{0.41 (0.23)} & \textbf{0.23 (0.18)} & \textbf{0.34 (0.14)} \\
% LASER & \multicolumn{1}{|c|}{0.24 \pm 0.17 (0.15 \pm 0.12)} & 0.62 (0.43) & 0.23 (0.18) & 0.02 (0.01) & 0.24 (0.14) & 0.33 (0.22) & 0.11 (0.06) & 0.39 (0.21) & 0.30 (0.17) & 0.06 (0.05) & 0.13 (0.05) \\
% S-BERT & \multicolumn{1}{|c|}{0.39 \pm 0.13 (0.24 \pm 0.11)} & 0.64 (0.46) & 0.53 (0.41) & 0.37 (0.22) & 0.30 (0.17) & 0.42 (0.28) & 0.31 (0.17) & 0.53 (0.29) & 0.31 (0.17) & 0.19 (0.14) & 0.31 (0.13) \\
% S-BERT XLM-R & \multicolumn{1}{|c|}{0.38 \pm 0.15 (0.24 \pm 0.12)} & 0.67 (0.47) & 0.55 (0.43) & 0.35 (0.20) & 0.29 (0.16) & 0.42 (0.27) & 0.28 (0.15) & 0.51 (0.27) & 0.29 (0.16) & 0.15 (0.12) & 0.28 (0.12) \\
% Hybrid XLM-R (k=64) & \multicolumn{1}{|c|}{0.43 \pm 0.14 (0.26 \pm 0.11)} & 0.69 (0.49) & \textbf{0.58 (0.45)} & \textbf{0.40 (0.23)} & 0.32 (0.18) & 0.46 (0.30) & \textbf{0.35 (0.20)} & \textbf{0.54 (0.29)} & 0.38 (0.21) & 0.20 (0.15) & 0.33 (0.13) \\\midrule


% Hybrid XLM-R (k=32) & \multicolumn{1}{|c|}{0.42 \pm 0.14 (0.26 \pm 0.12)} & 0.69 (0.49) & \textbf{0.58 (0.45)} & \textbf{0.40 (0.23)} & 0.32 (0.18) & 0.45 (0.30) & 0.34 (0.19) & \textbf{0.54 (0.29)} & 0.37 (0.21) & 0.19 (0.15) & 0.32 (0.13) \\
% Hybrid XLM-R (k=16) & \multicolumn{1}{|c|}{0.42 \pm 0.14 (0.26 \pm 0.12)} & 0.69 (0.49) & \textbf{0.58 (0.44)} & \textbf{0.40 (0.23)} & 0.31 (0.17) & 0.45 (0.30) & 0.33 (0.19) & \textbf{0.54 (0.29)} & 0.36 (0.19) & 0.18 (0.14) & 0.32 (0.13) \\
% Hybrid XLM-R (k=8) & \multicolumn{1}{|c|}{0.41 \pm 0.14 (0.25 \pm 0.12)} & 0.68 (0.49) & 0.57 (0.44) & 0.39 (0.23) & 0.31 (0.18) & 0.44 (0.29) & 0.32 (0.18) & 0.53 (0.29) & 0.34 (0.19) & 0.18 (0.13) & 0.31 (0.13) \\
% Hybrid XLM-R (k=4) & \multicolumn{1}{|c|}{0.40 \pm 0.14 (0.25 \pm 0.12)} & 0.68 (0.49) & 0.57 (0.44) & 0.38 (0.22) & 0.31 (0.17) & 0.44 (0.29) & 0.31 (0.18) & 0.53 (0.29) & 0.33 (0.18) & 0.17 (0.13) & 0.31 (0.13) \\
 
 
% NMT + USE & \multicolumn{1}{|c|}{0.39 (0.24)} & 0.68 (0.48) & 0.56 (0.43) & 0.46 (0.25) & 0.42 (0.28) & 0.39 (0.23) & 0.35 (0.20) & 0.33 (0.19) & 0.31 (0.17) & 0.19 (0.07) & 0.18 (0.14) \\\midrule
% mUSE & \multicolumn{1}{|c|}{0.32 (0.21)} & \textbf{0.70 (0.50)} & \textbf{0.58 (0.45)} & 0.12 (0.07) & \textbf{0.47 (0.31)} & 0.04 (0.03) & \textbf{0.41 (0.23)} & 0.02 (0.01) & \textbf{0.33 (0.19)} & \textbf{0.34 (0.14)} & \textbf{0.23 (0.18)} \\
% LASER & \multicolumn{1}{|c|}{0.24 (0.15)} & 0.62 (0.43) & 0.23 (0.18) & 0.39 (0.21) & 0.33 (0.22) & 0.02 (0.01) & 0.30 (0.17) & 0.11 (0.06) & 0.24 (0.14) & 0.13 (0.05) & 0.06 (0.05) \\
% S-BERT & \multicolumn{1}{|c|}{0.39 (0.24)} & 0.64 (0.46) & 0.53 (0.41) & 0.53 (0.29) & 0.42 (0.28) & 0.37 (0.22) & 0.31 (0.17) & 0.31 (0.17) & 0.30 (0.17) & 0.31 (0.13) & 0.19 (0.14) \\
% S-BERT XLM-R & \multicolumn{1}{|c|}{0.38 (0.24)} & 0.67 (0.47) & 0.55 (0.43) & 0.51 (0.27) & 0.42 (0.27) & 0.35 (0.20) & 0.29 (0.16) & 0.28 (0.15) & 0.29 (0.16) & 0.28 (0.12) & 0.15 (0.12) \\
% Hybrid XLM-R (k=64) & \multicolumn{1}{|c|}{\textbf{0.43 (0.26)}} & 0.69 (0.49) & \textbf{0.58 (0.45)} & \textbf{0.54 (0.29)} & 0.46 (0.30) & \textbf{\textbf{0.40 (0.23)}} & 0.38 (0.21) & \textbf{0.35 (0.20)} & 0.32 (0.18) & 0.33 (0.13) & 0.20 (0.15) \\\midrule



% TODO: Fix this
% \textit{Perfect XX $\rightarrow$ EN} & \multicolumn{1}{|c|}{0.47 \pm 0.13 (0.29 \pm 0.11)} & 0.87 (0.79) & 0.90 (0.85) & 0.89 (0.83) & 0.86 (0.77) & 0.90 (0.85) & 0.75 (0.65) & 0.75 (0.56) & 0.51 (0.45) & 0.65 (0.58) & 0.33 (0.32) \\

% xquad: 0.29 \pm 0.11 (0.47 \pm 0.13)
% mkqa: 0.76 \pm 0.18 (0.69 \pm 0.17)

\midrule
 & \multicolumn{4}{c}{MKQA + Natural Questions (WikiData)} \\
\cmidrule{2-5}
 & \multicolumn{1}{|c|}{avg} & High & Medium & Low \\
\midrule


NMT + USE & \multicolumn{1}{|c|}{0.69 $\pm$ 0.16 (0.66 $\pm$ 0.16)} & 0.74 $\pm$ 0.14 (0.71 $\pm$ 0.14) & 0.73 $\pm$ 0.11 (0.70 $\pm$ 0.11) & 0.53 $\pm$ 0.17 (0.48 $\pm$ 0.17) \\\hline
mUSE & \multicolumn{1}{|c|}{0.66 $\pm$ 0.19 (0.63 $\pm$ 0.18)} & \textbf{0.81} $\pm$ 0.08 (0.78 $\pm$ 0.09) & 0.54 $\pm$ 0.18 (0.53 $\pm$ 0.17) & 0.63 $\pm$ 0.16 (0.58 $\pm$ 0.16) \\
LASER & \multicolumn{1}{|c|}{0.68 $\pm$ 0.15 (0.65 $\pm$ 0.15)} & 0.65 $\pm$ 0.14 (0.63 $\pm$ 0.14) & \textbf{0.76} $\pm$ 0.10 (0.74 $\pm$ 0.09) & 0.56 $\pm$ 0.17 (0.52 $\pm$ 0.17) \\
S-BERT & \multicolumn{1}{|c|}{0.67 $\pm$ 0.08 (0.63 $\pm$ 0.08)} & 0.67 $\pm$ 0.04 (0.64 $\pm$ 0.05) & 0.68 $\pm$ 0.09 (0.65 $\pm$ 0.09) & 0.63 $\pm$ 0.07 (0.57 $\pm$ 0.08) \\
S-BERT XLM-R & \multicolumn{1}{|c|}{0.65 $\pm$ 0.11 (0.62 $\pm$ 0.11)} & 0.69 $\pm$ 0.07 (0.66 $\pm$ 0.08) & 0.66 $\pm$ 0.12 (0.63 $\pm$ 0.12) & 0.59 $\pm$ 0.10 (0.53 $\pm$ 0.11) \\
Hybrid XLM-R (k=64) & \multicolumn{1}{|c|}{\textbf{0.73} $\pm$ 0.09 (0.70 $\pm$ 0.10)} & 0.77 $\pm$ 0.07 (0.73 $\pm$ 0.08) & 0.74 $\pm$ 0.09 (0.71 $\pm$ 0.09) & \textbf{0.66} $\pm$ 0.09 (0.60 $\pm$ 0.10) \\
% Hybrid XLM-R (k=32) & \multicolumn{1}{|c|}{0.73 $\pm$ 0.09 (0.69 $\pm$ 0.10)} & 0.76 $\pm$ 0.07 (0.73 $\pm$ 0.08) & 0.74 $\pm$ 0.09 (0.71 $\pm$ 0.09) & 0.66 $\pm$ 0.09 (0.60 $\pm$ 0.10) \\
% Hybrid XLM-R (k=16) & \multicolumn{1}{|c|}{0.72 $\pm$ 0.10 (0.69 $\pm$ 0.10)} & 0.76 $\pm$ 0.07 (0.72 $\pm$ 0.08) & 0.73 $\pm$ 0.09 (0.70 $\pm$ 0.09) & 0.65 $\pm$ 0.10 (0.59 $\pm$ 0.10) \\
% Hybrid XLM-R (k=8) & \multicolumn{1}{|c|}{0.72 $\pm$ 0.10 (0.68 $\pm$ 0.10)} & 0.75 $\pm$ 0.07 (0.72 $\pm$ 0.08) & 0.72 $\pm$ 0.10 (0.70 $\pm$ 0.09) & 0.64 $\pm$ 0.10 (0.59 $\pm$ 0.10) \\
% Hybrid XLM-R (k=4) & \multicolumn{1}{|c|}{0.71 $\pm$ 0.10 (0.68 $\pm$ 0.10)} & 0.74 $\pm$ 0.07 (0.71 $\pm$ 0.08) & 0.72 $\pm$ 0.10 (0.69 $\pm$ 0.09) & 0.63 $\pm$ 0.10 (0.58 $\pm$ 0.10) \\
\midrule
\textit{Perfect XX $\rightarrow$ EN} & \multicolumn{1}{|c|}{0.76 \pm 0.18 (0.69 \pm 0.17)} & 0.79 $\pm$ 0.17 (0.71 $\pm$ 0.17) & 0.81 $\pm$ 0.11 (0.73 $\pm$ 0.11) & 0.59 $\pm$ 0.22 (0.53 $\pm$ 0.19) \\




% NMT + USE & \multicolumn{1}{|c|}{0.69 (0.66)} & \textbf{0.86 (0.83)} & 0.85 (0.82) & 0.84 (0.81) & 0.83 (0.80) & 0.84 (0.81) & 0.60 (0.58) & 0.60 (0.54) & 0.47 (0.46) & 0.45 (0.38) & 0.35 (0.32) \\\midrule
% mUSE & \multicolumn{1}{|c|}{0.66 (0.63)} & 0.50 (0.49) & 0.89 (0.85) & \textbf{0.88 (0.84)} & \textbf{0.89 (0.86)} & \textbf{0.87 (0.84)} & 0.69 (0.66) & \textbf{0.75 (0.69)} & \textbf{0.63 (0.61)} & 0.35 (0.32) & \textbf{0.56 (0.50)} \\
% LASER & \multicolumn{1}{|c|}{0.68 (0.65)} & 0.85 (0.82) & \textbf{0.90 (0.87)} & 0.75 (0.73) & 0.81 (0.78) & 0.51 (0.50) & \textbf{0.70 (0.68)} & 0.39 (0.36) & 0.59 (0.57) & 0.38 (0.36) & 0.46 (0.42) \\
% S-BERT & \multicolumn{1}{|c|}{0.67 (0.63)} & 0.81 (0.78) & 0.76 (0.73) & 0.71 (0.68) & 0.63 (0.60) & 0.72 (0.69) & 0.51 (0.49) & 0.68 (0.62) & 0.62 (0.60) & 0.55 (0.47) & 0.54 (0.49) \\
% S-BERT XLM-R & \multicolumn{1}{|c|}{0.65 (0.62)} & 0.82 (0.78) & 0.81 (0.78) & 0.75 (0.72) & 0.73 (0.70) & 0.77 (0.74) & 0.46 (0.45) & 0.63 (0.56) & 0.54 (0.52) & 0.49 (0.41) & 0.48 (0.44) \\
% Hybrid XLM-R (k=64) & \multicolumn{1}{|c|}{\textbf{0.73 (0.70)}} & 0.85 (0.82) & 0.85 (0.82) & 0.82 (0.79) & 0.82 (0.78) & 0.83 (0.80) & 0.59 (0.57) & 0.72 (0.66) & 0.61 (0.59) & \textbf{0.59 (0.51)} & 0.55 (0.49) \\\midrule

%  & \multicolumn{1}{|c|}{avg} & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ \\
% \midrule
% NMT + USE & \multicolumn{1}{|c|}{\_\_} & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ \\\hline
% \_\_ & \multicolumn{1}{|c|}{\_\_} & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ \\
% \_\_ & \multicolumn{1}{|c|}{\_\_} & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ \\
% \_\_ & \multicolumn{1}{|c|}{\_\_} & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ & \_\_ \\\hline
% \textit{Perfect XX $\rightarrow$ EN} & \multicolumn{1}{|c|}{0.76 \pm 0.18 (0.69 \pm 0.17)} & 0.87 (0.79) & 0.90 (0.85) & 0.89 (0.83) & 0.86 (0.77) & 0.90 (0.85) & 0.75 (0.65) & 0.75 (0.56) & 0.51 (0.45) & 0.65 (0.58) & 0.33 (0.32) \\

% \bottomrule
% \toprule
%  & \multicolumn{10}{c}{MKQA} \\
% \cmidrule{2-13}
%  & \multicolumn{1}{|c}{avg} & \multicolumn{1}{c|}{std} & ar & da & de & es & fi & fr & he & hu & it & ja\\
% \midrule
% NMT USE-L & \multicolumn{1}{|l}{0.82} & \multicolumn{1}{l|}{0.093} & 0.80 & \textbf{0.95} & 0.94 & 0.93 & 0.86 & 0.94 & 0.85 & 0.89 & 0.93 & 0.75 \\\hline
% LASER & \multicolumn{1}{|l}{0.79} & \multicolumn{1}{l|}{0.260} & \textbf{0.90} & 0.93 & 0.58 & 0.87 & 0.89 & 0.86 & \textbf{0.92} & 0.78 & 0.87 & 0.51 \\
% MUSE-L & \multicolumn{1}{|l}{0.51} & \multicolumn{1}{l|}{0.395} & 0.89 & 0.65 & \textbf{0.96} & \textbf{0.97} & 0.48 & \textbf{0.96} & 0.32 & 0.51 & \textbf{0.96} & \textbf{0.89} \\
% XLM-R & \multicolumn{1}{|l}{\textbf{0.91}} & \multicolumn{1}{l|}{\textbf{0.014}} & 0.83 & \textbf{0.95} & 0.93 & \textbf{0.94} & \textbf{0.91} & 0.92 & 0.89 & \textbf{0.90} & 0.92 & 0.88 \\
% SBERT XLM-R & \multicolumn{1}{|l}{0.85} & \multicolumn{1}{l|}{0.057} & 0.63 & 0.92 & 0.88 & 0.88 & 0.76 & 0.87 & 0.73 & 0.78 & 0.83 & 0.77 \\
% Hybrid XLM-R & \multicolumn{1}{|l}{\textbf{0.91}} & \multicolumn{1}{l|}{\textbf{0.014}} & 0.78 & \textbf{0.95} & 0.93 & 0.93 & 0.88 & 0.93 & 0.87 & 0.88 & 0.91 & 0.87 \\
\bottomrule

\end{tabular}
\end{small}}
\caption{End-To-End F1 and EM: The average F1 (EM) scores obtained for each method when mapping from queries in a given language to English then back to the original language. We use a Many-to-Many NMT to generate the language in the original langauge for XQuAD, and WikiData translation for MKQA. For reference, \textit{Perfect XX $\rightarrow$ EN} shows the results obtained when using the ground truth English answer in back translation. Only a subset of the MQKA langauge results are shown: 5 of the languages NMT + USE performs the best, and 5 which it's least performant. Averages are across all languages in the dataset.}
\end{table*}


%  & \multicolumn{1}{|c|}{avg} & es & de & vi & tr & el & ar & hi & ru & zh & th \\
% \midrule
% NMT + USE & \multicolumn{1}{|c|}{0.39 (0.24)} & 0.68 (0.48) & 0.56 (0.43) & 0.46 (0.25) & 0.42 (0.28) & 0.39 (0.23) & 0.35 (0.20) & 0.33 (0.19) & 0.31 (0.17) & 0.19 (0.07) & 0.18 (0.14) \\
% mUSE & \multicolumn{1}{|c|}{0.32 (0.21)} & \textbf{0.70 (0.50)} & \textbf{0.58 (0.45)} & 0.12 (0.07) & \textbf{0.47 (0.31)} & 0.04 (0.03) & \textbf{0.41 (0.23)} & 0.02 (0.01) & \textbf{0.33 (0.19)} & \textbf{0.34 (0.14)} & \textbf{0.23 (0.18)} \\
% LASER & \multicolumn{1}{|c|}{0.24 (0.15)} & 0.62 (0.43) & 0.23 (0.18) & 0.39 (0.21) & 0.33 (0.22) & 0.02 (0.01) & 0.30 (0.17) & 0.11 (0.06) & 0.24 (0.14) & 0.13 (0.05) & 0.06 (0.05) \\
% S-BERT & \multicolumn{1}{|c|}{0.39 (0.24)} & 0.64 (0.46) & 0.53 (0.41) & 0.53 (0.29) & 0.42 (0.28) & 0.37 (0.22) & 0.31 (0.17) & 0.31 (0.17) & 0.30 (0.17) & 0.31 (0.13) & 0.19 (0.14) \\
% S-BERT XLM-R & \multicolumn{1}{|c|}{0.38 (0.24)} & 0.67 (0.47) & 0.55 (0.43) & 0.51 (0.27) & 0.42 (0.27) & 0.35 (0.20) & 0.29 (0.16) & 0.28 (0.15) & 0.29 (0.16) & 0.28 (0.12) & 0.15 (0.12) \\
% Hybrid XLM-R (k=64) & \multicolumn{1}{|c|}{0.43 (0.26)} & 0.69 (0.49) & \textbf{0.58 (0.45)} & \textbf{0.54 (0.29)} & 0.46 (0.30) & \textbf{0.40 (0.23)} & 0.38 (0.21) & \textbf{0.35 (0.20)} & 0.32 (0.18) & 0.33 (0.13) & 0.20 (0.15) \\
% Hybrid XLM-R (k=32) & \multicolumn{1}{|c|}{0.42 (0.26)} & 0.69 (0.49) & \textbf{0.58 (0.45)} & \textbf{0.54 (0.29)} & 0.45 (0.30) & \textbf{0.40 (0.23)} & 0.37 (0.21) & 0.34 (0.19) & 0.32 (0.18) & 0.32 (0.13) & 0.19 (0.15) \\
% Hybrid XLM-R (k=16) & \multicolumn{1}{|c|}{0.42 (0.26)} & 0.69 (0.49) & \textbf{0.58 (0.44)} & \textbf{0.54 (0.29)} & 0.45 (0.30) & \textbf{0.40 (0.23)} & 0.36 (0.19) & 0.33 (0.19) & 0.31 (0.17) & 0.32 (0.13) & 0.18 (0.14) \\
% Hybrid XLM-R (k=8) & \multicolumn{1}{|c|}{0.41 (0.25)} & 0.68 (0.49) & 0.57 (0.44) & 0.53 (0.29) & 0.44 (0.29) & 0.39 (0.23) & 0.34 (0.19) & 0.32 (0.18) & 0.31 (0.18) & 0.31 (0.13) & 0.18 (0.13) \\
% Hybrid XLM-R (k=4) & \multicolumn{1}{|c|}{0.40 (0.25)} & 0.68 (0.49) & 0.57 (0.44) & 0.53 (0.29) & 0.44 (0.29) & 0.38 (0.22) & 0.33 (0.18) & 0.31 (0.18) & 0.31 (0.17) & 0.31 (0.13) & 0.17 (0.13) \\


%  & XQuAD (NMT) & MKQA (WikiData) \\
% \midrule
% el&0.26 (0.45)&-(-)\\
% hi&0.23 (0.40)&-(-)\\
% ru&0.20 (0.35)&0.71 (0.65)\\
% de&0.47 (0.61)&0.90 (0.85)\\
% ar&0.26 (0.46)&0.75 (0.65)\\
% zh&0.15 (0.37)&-(-)\\
% th&0.19 (0.25)&0.73 (0.61)\\
% es&0.51 (0.71)&0.90 (0.84)\\
% tr&0.32 (0.50)&0.87 (0.79)\\
% vi&0.31 (0.58)&0.86 (0.77)\\
% zh-tw&-(-)&0.33 (0.32)\\
% ko&-(-)&0.51 (0.45)\\
% no&-(-)&0.88 (0.82)\\
% zh-hk&-(-)&0.34 (0.32)\\
% pl&-(-)&0.84 (0.76)\\
% hu&-(-)&0.85 (0.77)\\
% ja&-(-)&0.75 (0.56)\\
% he&-(-)&0.75 (0.64)\\
% it&-(-)&0.89 (0.84)\\
% nl&-(-)&0.90 (0.85)\\
% fi&-(-)&0.84 (0.77)\\
% ms&-(-)&0.89 (0.83)\\
% zh-cn&-(-)&0.33 (0.32)\\
% km&-(-)&0.65 (0.58)\\
% pt&-(-)&0.86 (0.77)\\
% fr&-(-)&0.89 (0.83)\\
% da&-(-)&0.87 (0.79)\\
% sv&-(-)&0.86 (0.78)\\
% \bottomrule

% xquad: 0.29 (0.47)
% mkqa: 0.76 (0.69)

% 0.87 (0.79) & 0.90 (0.85) & 0.89 (0.83) & 0.86 (0.77) & 0.90 (0.85) & 0.75 (0.65) & 0.75 (0.56) & 0.51 (0.45) & 0.65 (0.58) & 0.33 (0.32)


% Overall
% xquad: 0.29 \pm 0.11 (0.47 \pm 0.13)
% mkqa: 0.76 \pm 0.18 (0.69 \pm 0.17)
% ====== GROUPS ======
%  & High & Medium & Low
% XQuAD  & 0.33 $\pm$ 0.16 (0.51 $\pm$ 0.16) & 0.30 $\pm$ 0.03 (0.51 $\pm$ 0.05) & 0.23 $\pm$ 0.03 (0.36 $\pm$ 0.08)
% MKQA & 0.79 $\pm$ 0.17 (0.71 $\pm$ 0.17) & 0.81 $\pm$ 0.11 (0.73 $\pm$ 0.11) & 0.59 $\pm$ 0.22 (0.53 $\pm$ 0.19)
% ====== LANGUAGE TABLE ======
%  & XQuAD & MKQA \\
% High & es, de, ru, zh & de, es, zh_cn, ru, pl, fr, pt, ja, it
% Medium & vi, ar, tr & vi, da, ar, ko, tr, nl, hu, no, fi, he, sv
% Low & hi, el, th & ms, zh_tw, th, km, zh_hk
